Emulating duration and curvature of coral snake anti-predator thrashing behaviors using a soft-robotic platform

This paper presents a soft-robotic platform for exploring the ecological relevance of non-locomotory movements via animal-robot interactions. Coral snakes (genus Micrurus) and their mimics use vigorous, non-locomotory, and arrhythmic thrashing to deter predation. There is variation across snake species in the duration and curvature of anti-predator thrashes, and it is unclear how these aspects of motion interact to contribute to snake survival. In this work, soft robots composed of fiber-reinforced elastomeric enclosures (FREEs) are developed to emulate the anti-predator behaviors of three genera of snake. Curvature and duration of motion are estimated for both live snakes and robots, providing a quantitative assessment of the robots' ability to emulate snake poses. The curvature values of the fabricated soft-robotic head, midsection, and tail segments are found to overlap with those exhibited by live snakes. Soft robot motion durations were less than or equal to those of snakes for all three genera. Additionally, combinations of segments were selected to emulate three specific snake genera with distinct anti-predatory behavior, producing curvature values that aligned well with live snake observations.

==> sections/00_outline.tex <==
\section{Outline}
\Dan{This is the rough outline I wrote down in our meeting but please amend as needed.}

\begin{enumerate}
    \item Introduction
        \begin{itemize}
            \item Talia: ``Soft robots aren't yet controllable enough to perform the same tasks as rigid robots, but they can enable biological experiments that would have previously been impossible.''
        \end{itemize}
    \item Design and Fabrication
        \begin{itemize}
            \item Dan: Describe theory of cylindrical volumes with strain limiting layers.
            \item Maggie: Describe fabrication of snakes.
            \item Figures: Diagram to illustrate volume expansion with strain limiting fiber reinforcements, photos showing the various fabrication steps.
        \end{itemize}
    \item Experiments / Results
        \begin{itemize}
            \item Talia: Describe how data was collected on real snakes.
            \item Shannon: Describe method for quantifying shape/curvature.
            \item Shannon: Quantify/compare curvature of real snakes and robot snakes.
            \item Figures: Side-by-side pictures of real/robot snakes, plot(s) to show quantitative curvature results.
        \end{itemize}
    \item Conclusion
        \begin{itemize}
            \item Talia: Reverse the order of sentences from the introduction :)
        \end{itemize}
\end{enumerate}
